Talking to Machines: do you read me?

In this dissertation I would like to guide the reader to the research on dialogue but more precisely the research I have conducted during my career since my PhD thesis. Starting from modular architectures with machine learning/deep learning and reinforcement learning to end-to-end deep neural networks. Besides my work as research associate, I also present the work I have supervised in the last years. I review briefly the state of the art and highlight the open research problems on conversational agents. Afterwards, I present my contribution to Task-Oriented Dialogues (TOD), both as research associate and as the industrial supervisor of CIFRE theses. I discuss conversational QA. Particularly, I present the work of two PhD candidates Thibault Cordier and Sebastien Montella; as well as the work of the young researcher Quentin Brabant. Finally, I present the scientific project, where I discuss about Large Language Models (LLMs) for Task-Oriented Dialogue and Multimodal Task-Oriented Dialogue.

==> chap5.tex <==
\chapter{Curriculum Vitae}
\label{c:cv}

\section{\large \scshape {Academic Background}}
%\cventry{1000--2000}{Degree}{Institution}{City}{\textit{Grade}}{Description}

\cventry{2005--2009}{Ph.D. in Biotechnology and Bioinformatics}{Università degli Studi di Pavia}{Italy}{Thesis: Health Care Dialogue Systems: Practical and Theoretical Approaches to Dialogue Management. Advisor: Prof. Mario Stefanelli Dissertation Date:  17 February 2009.}{}{}
%Thesis: Health Care Dialogue Systems: Practical and Theoretical Approaches to Dialogue Management
%Advisor: Mario Stefanelli Dissertation Date: February 17 2009
\noindent \cventry{2004--2005}{Master's degree (MSc)  in Software Engineering}{Universidad Polit\'{e}cnica de Madrid}{Spain}{}{}
%{Thesis: Application of Software engineering principles in a real software project applied to the Laboratory for Proteomics at the CNB (Madrid).}

\noindent \cventry{1993--1999}{Degree in Systems Engineering}{Universidad del Valle}{Cali Colombia}{(5-year engineering degree)}{}
%{Thesis: Design and Development of a Content-Based Image Retrieval System, which allows queries by color, shape, edges and patterns by using and object oriented database.}
 

%\vspace{0.5cm}

%\section*{\large \scshape {Tecnical Skills and Competences}}

%\begin{itemize}
% \item[] \textbf{Machine Learning}: Deep, Supervised, Unsupervised and Reinforcement Learning. Tools: Octave, R, MALLET, Stanford Classifier, Stanford NER, WEKA, Deeplearning4j and Theano.\vspace{0.15cm}
% \item[] \textbf{Natural Language Processing}: NLU, Dialogue Systems, NLG, Corpus Annotation. Tools: StanfordCoreNLP, NLTK, MALT, MATE, Stanford and Tweebo Parsers.\vspace{0.15cm}
% \item[] \textbf{Computational Linguistics}: Formal Grammars and First Order Logic. Tools: Combinatory Categorial Grammars, Description Logics and Dependency Trees.\vspace{0.15cm}. Tools: OpenCCG, Protégé and RACER.
% \item[] \textbf{Programming Languages}: JAVA, Python, C, C++, ORACLE PL/SQL, VisualBasic.\vspace{0.15cm} Web development, databases and software best practices.
% \item[] \textbf{WEB}: HTML, Javascript, JSP, GWT, Apache Struts, Enterprise Java Beans and Spring.\vspace{0.15cm}
 %\item[] \textbf{Databases}: SQL, OQL, ORACLE 9i, ORACLE PL/SQL and toolkits, mysql, POET OODBMS , JDBC and Hibernate. \vspace{0.15cm}
 %\item[] \textbf{Software Best Practices}:  UML, XML, XSLT, TEI, VoiceXML et SRGS grammars.
%\end{itemize} 
   
 \section*{\large \scshape {Languages}}
%(455 TFI)
%\begin{tabular}{ccccc}
\textbf{Spanish}: Native speaker; \textbf{English}, \textbf{French} and \textbf{Italian}: Fluent; \textbf{Portuguese}: Basic level.
%\end{tabular} 
  
%\section*{\large \scshape \textcolor{blue}{Trainings}}
%
%\cvitem{09/2017}{EMNLP Tutorial : \textbf{Memory Augmented Neural Networks for NLP}. Tutors: Caglar Gulcehre and Sarath Chandar. Copenhagen, Denmark}
%\cvitem{08/2013}{Statement of accomplishment of the on-line course: \textbf{Model Thinking}. Professor Scott E. Page. University of Michigan. Coursera.}
%\cvitem{07/2011}{ACL Tutorial 2011: \textbf{Beyond Structured Prediction: Inverse Reinforcement Learning}. Professor: Hal Daume III, University of Maryland. Portland Oregon.}
%\cvitem{11/2011}{Statement of accomplishment of the on-line \textbf{ Machine Learning course}. Professor Andrew Ng. University of Stanford. Coursera}
%\cvitem{09/2008}{Summer school on \textbf{Bioengineering and Bioinformatics}. Bressanone, Italy}
%\cvitem{09/2007}{Research Internship on NLP , \textbf{Natural Language Processing}. Professor: Patrick Blackburn. Talaris team at LORIA. Nancy, France.}
%\cvitem{07/2007}{Participation at the doctoral consortium at AIME07  (\textbf{Artificial Intelligence in Medicine}).}
%\cvitem{09/2006}{Summer school on \textbf{Bioengineering and Bioinformatics}. Bressanone, Italy}
%\cvitem{09/2006}{Summer School on \textbf{The Fundamentals of Verbal and Non-verbal Communication and the Biometrical Issue.} Vietri, Italy.}
 
 
 
%\section*{\large \sc Academic and Industrial Experience}
\section*{\large  \scshape {Research Experience}}

%\cventry{year--year}{Job title}{Employer}{City}{}{Description line 1\newline{}Description line 2}

\cventry{2018-- now}{Researcher in statistical spoken dialogue systems.}{Orange Innovation}{France}{}{Researcher on dialogue systems, head of the workpackage \ac{TOD} of the research project LANGUAGE from 2023 on. Head of Orange's research project \ac{DIANA} (2018-2023); co-supervisor of four PhD thesis on open dialogue systems, hierarchical imitation learning, generation and \ac{DST}; supervisor of internships and apprenticeships on dialogue.}
\noindent \cventry{2015--2018}{Research associate in open-domain statistical spoken dialogue systems.}{Department of Engineering at the University of Cambridge}{UK}{}{Researcher on deep \ac{SLU}, scalable to multiple domains and for cognitive behavioural therapy. Contributed to PyDial statistical dialogue framework. Designed the voice communication protocol between PyDial dialogue server and Voice Clients. Contributed to the implementation of the VoiceBroker: interfacing \ac{VoIP} with available \ac{ASR} APIs and \ac{TTS}.}
\noindent \cventry{2014--2015}{Universit\'e de Lorraine postdoctoral researcher.}{Projects Empathic (Sentiment Analysis) and  ContNomina (Named Entity Recognition from speech transcriptions).}{Synalp team at LORIA.}{Nancy France}{Experimented with recursive neural networks for dependency trees on Twitter and formulated and applied unsupervised learning of discriminative models.}
\noindent \cventry{2012--2014}{ATER (Temporary professor and researcher).}{Universit\'e de Lorraine.}{Synalp team at LORIA.}{Nancy France}{Conducted research on Inverse Reinforcement Learning. Participated in science communication events.}
\noindent \cventry{2010--2012}{INRIA postdoctoral position.}{Eurostar Project: Emospeech, integrating conversational agents in serious games.}{Talaris team at LORIA.}{Nancy France}{Research on symbolic and statistical end-to-end dialogue systems. Achieved the implementation and evaluation of distinct dialogues. Organised workshops and participated in science communication events.}
\noindent \cventry{2009--2010}{CNRS postdoctoral position.}{ANR Project: PortMedia, automatic semantic annotation of dialogue corpora.}{Talaris team at LORIA.}{Nancy France}{Formalised the semantics and achieved the automatic semantic annotation of the MEDIA corpus.}
%% \textbf{2009} &Postdoctoral fellowship. Research in clinical NLP applications.  Laboratory for Biomedical Informatics. Universit\`{a} degli Studi di Pavia, Italy.\\&\\
\noindent \cventry{2005--2009}{Research in health-care dialogue systems.}{Laboratory for Biomedical Informatics.}{Postdoctoral fellowship and Ph.D. student}{Universit\`{a} degli Studi di Pavia. Italy}{Main contributor to AdaRTE, a health-care dialogue framework and creator of HomeNL, homecare in natural language.}{}
\noindent \cventry{2004--2005}{Bionformatics support engineer.}{Laboratory of Proteomics and PROTEORED. }{Predoctoral scholarship}{Centro Nacional de Biotecnolog\'{i}a (CNB)} {Madrid Spain.}
% %\textbf{2003} &Research collaborator. Topics: classification of mammographies by using support vector machine and web-based application for querying diagnosis and retrieving medical images based on content. \\& Universidad del Valle, Cali Colombia.\\&\\
%%\textbf{1996-1997}&Programmer in a project of coordination of independent\\& circular bodies movement inside polygonal walls.\\& Universidad del Valle, Cali, Colombia.
     

\section*{\large  \scshape {Industrial Experience}}

 \noindent \cventry{2000--2004}{Team leader, software analyst and developer.}{Open International Systems (Oracle Partner)}{Cali Colombia.}{Software for business and critical-operations, addressed to telecommunications and public service companies.}{}
% \begin{itemize}
%  \item Leader of the Customize Team, in charge of custom-made software for the products: OpenflexIs 4.0, Gestel Plus and SATPlus.
% \item Developer for OpenflexIs5.0, OpenflexIs4.0 and Gestel Plus. 
% \item Developer in the Sercomtel team, the Open-Sercomtel Project for OpenflexIs4.0. Brazil (2000-2001).
% \end{itemize}\\

 \noindent \cventry{1998--1999}{Freelancer.}{Developer of software for Human Resources Management}{Gillette Colombia S.A}{Cali Colombia.}{}

%\section*{\large \sc Teaching and Co-supervision of Students}

\section*{\large \scshape {Teaching Experience}}
\cventry{2018--2022}{Lecturer of Introduction to Dialogue Systems.}{ENSSAT, Université de Rennes 1}{Lannion}{France}{}
\noindent \cventry{2021}{Lecturer of Introduction to Dialogue Systems. Ecole d'été en TAL}{ENSSAT, Université de Rennes 1}{Lannion}{France}{}
\noindent \cventry{2018--2023}{Co-supervision of PhD and undergraduate students.}{Orange}{Lannion}{France}{}
\noindent \cventry{2016--2017}{Co-supervision of undergraduate students.}{University of Cambridge}{Cambridge}{UK}{}
 \noindent \cventry{2012--2013}{Lecturer (ATER)}{UFR Math\'ematique-Informatique, Universit\'e de Lorraine.}{Nancy France}{Courses: UML, Corpus Linguistics and Ing\'enierie des Langues (i.e., Natural Language Processing (NLP))}{ 
 Tutor of:  %(C2i) Certificat Informatique et Internet (i.e., Informatics and Internet certificate), 
 Tools for NLP, Initiation au Traitement Automatique des Langues (i.e. Introduction to NLP) and JAVA.Co-supervision of undergraduate students.}
 \noindent \cventry{2010--2012}{Tutor of Software Project in NLP, Master TAL Erasmus Mundus.}{LORIA-Universi\'e de Lorraine.} {Tutor of JAVA "Informatique 2" à l'Ecole des Mines, TD-TP. \newline{} Co-supervision of undergraduate students. }{Nancy France}{}
\noindent \cventry{2008-2009}{Co-supervision of graduate and undergraduate students.}{Universit\`{a} degli Studi di Pavia.}{Italy}{}{}
\noindent \cventry{1995--1998}{Undergraduate tutor of the courses of Compilers, Object-Oriented Databases and Computer Vision.}{Universidad del Valle}{Cali Colombia.}{}{}

\section*{\large \scshape{Serving as Jury}}
 \cvitem{\textbf{2020}} {Jury for the European projects ChisEra, call 2019 on Explainable Machine Learning-based Artificial Intelligence, \textbf{CHIST-ERA} supported by the Horizon 2020 FET programme of the EU}

\noindent \cvitem{\textbf{2019}} {Member of the jury of the PhD dissertation: Reinforcement learning for Dialogue Systems optimization with user adaptation.PhD Candidate: Nicolas Carrara. Supervisor: Olivier Pietquin. Université de Lille.France}

\noindent \cvitem{\textbf{2013}}{On the Jury of a Ph.D. Dissertation
: “Definition and Implementation of a controlled language for automatically characterizing informal argumentations”. PhD student : Raul Gutierrez de Pinerez. Supervisor : Juan Francisco Diaz Frias.
Universidad del Valle. Cali Colombia.}

\section*{\large \scshape {Complementary Activities}}
\cvitem{\textbf{2023}} {Reviewer for the journal Computer Speech \& Language. }.
\noindent \cvitem{\textbf{2018}--\textbf{2023}} {Reviewer for the conferences and workshops of the conferences: European Chapter of the Association for Computational Linguistics (\textbf{EACL}), Association for Computational Linguistics (\textbf{ACL}), Empirical Methods on Natural Language Processing (\textbf{EMNLP}), the North American Chapter of the Association for Computational Linguistics (\textbf{NAACL}), International Conference on Computational Linguistics (\textbf{COLING}) and  on Artificial Intelligence, (\textbf{AAAI})}.

\noindent \cvitem{\textbf{2017}}{Reviewer for the Empirical Methods on Natural Language Processing, \textbf{EMNLP} Copenhagen, Denmark.\newline{}
Reviewer for the Int. J. of Business Intelligence and Data Mining \textbf{IJBIDM}.}
\noindent \cvitem{\textbf{2016}}{Reviewer for the 26th International Conference on Computational Linguistics. \textbf{COLING}, Osaka Japan.}
\cvitem{}{Reviewer for the 29th Conference on Advances in Neural Information Processing Systems , \textbf{NIPS}, Barcelona Spain.}

\noindent \cvitem{\textbf{2012}}{Co-organiser of a workshop for collecting French dialogues for the integration of conversational agents in serious games. Loria, Artefacto and Ecole des beaux-arts de Rennes, France.
}
\noindent \cvitem{\textbf{2011}}{Member of \emph{The 7th Young Researchers' Roundtable on Spoken Dialogue Systems} (YRRSDS) organizing committee. Portland Oregon 2011.}
\noindent \cvitem{\textbf{2009}}{Reviewer for the 12th Conference on Artificial Intelligence in Medicine, \textbf{AIME}, Verona Italy.}
\noindent \cvitem{\textbf{2007}}{Reviewer for the 11th Conference on Artificial Intelligence in Medicine, \textbf{AIME}, Amsterdam, The Netherlands.}

%\section*{\large \sc Participation as  Organizer}
%\begin{tabular}{lp{15cm}}
%\textbf{2011}& Member of \emph{The 7th Young Researchers' Roundtable on Spoken Dialogue Systems} (YRRSDS) organizing committee. Portland Oregon 2011.  \url{http://www.yrrsds.org/}
%\end{tabular}
% \subsection*{Conferences}
% \begin{tabular}{lp{10cm}}
% \textbf{2012} & The eighth international conference on Language Resources and Evaluation. , May 2012, Istanbul, Turkey.\\&\\
% \textbf{2011} &The 49th Annual Meeting of the Association for Computational Linguistics: Human Language Technologies\\&\\
%  &12th annual SIGdial Meeting on Discourse and Dialogue. SIGDIAL 2011, Portland Oregon. June 2011\\&\\
% \textbf{2009} &12th Conference on Artificial Intelligence in Medicine (AIME 09), Verona Italy.\\&\\
% \textbf{2008}& XXVII Scuola di Bioingegneria organizzata dal GNB (Gruppo Nazionale di Bioingegneria). Il  Sistemi Indossabili Intelligenti per la Salute e la Protezione dell’Uomo. Bressanone, Italy\\&\\
% \textbf{2007}& 12th World Congress on Health (Medical) Informatics (MEDINFO 2007). Brisbane, Australia.\\&\\
% & 11th Conference on Artificial Intelligence in Medicine (AIME 07). Amsterdam, The Netherland.\\&\\
% & Workshop on the Semantics and Pragmatics of Dialogue (DECALOG2007). Rovereto, Italy.\\&\\
% \textbf{2006}&  XXV Suola Annuale di Bioingegneria organizzata dal GNB (Gruppo Nazionale di Bioingegneria). Neuro-Robotica: Neuorscienze e Robotica per lo sviluppo di machine intelligenti. Bressanone,  Italy.
%  \\&\\
%  & Summer School: The Fundamentals of Verbal and Non-verbal Communication and the Biometrical Issue. NATO Advanced Study Institute (ASI) University of Naples, University of Salerno and  International Institute for Advanced Scientific Studies, (IIASS). Vietri sul mare,  Italy.
%  \\&\\
% \textbf{2004} & Workshop on applications in proteomics 2004. CNB. Madrid Spain.
% \end{tabular}
% 

% \end{tabular}
% \subsection*{Participation as Organizer}
% \begin{tabular}{lp{10cm}}
% \textbf{2011}& Member of \emph{The 7th Young Researchers' Roundtable on Spoken Dialogue Systems} (YRRSDS) organizing committee. Portland Oregon 2011.  \url{http://www.yrrsds.org/}
% \end{tabular}
% \subsection*{Scientific talks}
% \begin{tabular}{lp{10cm}}
% \textbf{2012} &Building and Exploiting a Corpus of Dialog Interactions between French Speaking Virtual and Human Agents. LREC 2012, The eighth international conference on Language Resources and Evaluation. , May 2012, Istanbul, Turkey.\\&\\
% \textbf{2009} &HomeNL: Homecare Assistance in Natural Language. An Intelligent Conversational Agent for Hypertensive Patients Management. 12th Conference on Artificial Intelligence in Medicine, AIME09. Verona. Italy.\\&\\
%  \textbf{2008} &Dialogue systems in health (theoretical and functional approaches). Universit\`{a} degli Studi di Pavia. Italy.\\&\\
% \textbf{2007} &A framework for health-care dialogue systems.\\& Talaris team. Loria 2007. Nancy, France.\\&\\
%  &Adaptable dialogue architecture and runtime engine. A new architecture for health-care dialogue systems.\\&  12th World Congress on Health (Medical) Informatics (MEDINFO 2007). Brisbane Australia.\\&\\
%  &Adapting combinatory categorial grammars and knowledge-based features in a framework for health care dialogue systems. Doctoral consortium 11th Conference on Artificial Intelligence in Medicine (AIME 07). Amsterdam, The Netherlands.\\&\\
% \textbf{2006} &Software engineering best practices. Universit\`{a} degli Studi di Pavia. Italy.\\&\\
% \textbf{1995} &Automatic-generation of 3-D surfaces, student work on computater vision. Primer Encuentro Regional de Estudiantes de Ingeniería de Sistemas. Universidad del Valle. Cali, Colombia.
% \end{tabular}

\section*{\large \scshape {Awards and Scholarships}}
 \cvitem{\small{Best Student Paper Award}}{for the paper "On-line Active Reward Learning for Policy Optimisation in Spoken Dialogue Systems." ACL 2016}
 \cvitem{\small{Internship}}{NLP and Dialogue Systems, LORIA 2007.}
 \noindent \cvitem{\small{ISCA grant}}{Grant for attending the Summer School: The Fundamentals of Verbal and Non-verbal Communication and the Biometrical Issue. Vietri, Italy 2006 .}
 \noindent \cvitem{\small{Ph.D}}{Doctoral Scholarship, Italian Government 2005.}
 \noindent \cvitem{\small{Master}}{Pre-doctoral Scholarship, The Spanish National Research Council (CSIC) 2004.}   




%%
\section*{\large \scshape{Research Released Software}}
\begin{itemize}
\normalsize{
\item{\textbf{CoQAR}: Question Rewriting for Conversational Question Answering. } 
\item{\textbf{PyDial}: The Cambridge University Python Multi-domain Statistical Dialogue System Toolkit. }  \scriptsize{\url{https://www.camdial.org/pydial/}}\\
\item{\normalsize{\textbf{DLSemI}: Deep Learning for semantic decoding of dialogue systems (CNN,LSTM).} }  \scriptsize{\url{https://arxiv.org/abs/1610.04120}}\\
\item{\normalsize{\textbf{empathicLearning}: Recursive Neural Networks for sentiment analysis. }} 
\scriptsize{\url{http://synalp.loria.fr/pages/projects/}}\\
\item{\normalsize{\textbf{Contomina}: Supervised and unsupervised entity recognition. }} 
\scriptsize{\url{https://github.com/synalp/NER}}\\
\item{\normalsize{\textbf{Emospeech}: Dialogue system and toolkits for  semantic annotation of dialogue. }} 
\scriptsize{\url{http://synalp.loria.fr/pages/projects/}}\\
\item{\normalsize{\textbf{HLS}:  Framework for the semantic annotation of Portmedia corpus. }} 
\scriptsize{\url{http://sigdial.org/workshops/conference12/proc/pdf/SIGDIAL201139.pdf}}\\
\item{\normalsize{\textbf{HomeNL}: Homecare in natural language.}} 
\scriptsize{\url{http://www.labmedinfo.org/projects/HomeNL}}
\item{\normalsize{\textbf{\ac{AdaRTE}}: Framework for rapid prototyping of dialogue systems.} } 
\scriptsize{\url{http://www.labmedinfo.org/projects/adarte}}.
}
\end{itemize}
\section*{\large \scshape{Publications}}
\subsection{Journals}
\cvitem{2023}{\scriptsize{Michele Cafagna, Lina Rojas-Barahona, Kees van Deemter and Albert Gatt. \textbf{\em{Interpreting vision and language generative models with semantic visual priors}.} \textbf{Frontiers in Artificial Intelligence. }}}
\noindent\cvitem{2017}{\scriptsize{Milica Gašić, Nikola Mrkšić, Lina M. Rojas-Barahona, Pei-Hao Su, Stefan Ultes, David Vandyke, Tsung-Hsien Wen and Steve Young. \textbf{\em{Dialogue manager domain adaptation using Gaussian process reinforcement learning}.} \textbf{Computer Speech and Language},  45(5):552-569.}}

\noindent \cvitem{2016}{\scriptsize{Lina Maria Rojas-Barahona. \textbf{\em{Deep Learning for Sentiment Analysis.} Language and Linguistics Compass.} 10.12 (2016): 701-719.}}

\noindent \cvitem{2011}{\scriptsize{Bretaudi{\`e}re, Treveur and Cruz-Lara, Samuel and Rojas Barahona, Lina Maria. \textbf{\em{Associating Automatic Natural Language Processing to Serious Games and Virtual Worlds.} \textbf{The Journal of Virtual Worlds Research. Inc}, 2011, MPEG-V and Other Standards, 4 (3).}}}
\noindent \cvitem{2009}{\scriptsize{L.M. Rojas-Barahona, T. Giorgino. \textbf{\em{Adaptable dialog architecture and runtime engine (AdaRTE): A framework for rapid prototyping of health dialog systems.}} \textbf{International Journal of Medical Informatics}. Medinfo2007 Special Issue. vol. 78s ,pag. 56 - 68, (2009)}}

\subsection{Conferences }
%Kejriwal, Jay & Benus, Stefan & Rojas-Barahona, Lina. (2023). Unsupervised Auditory and Semantic Entrainment Models with Deep Neural Networks. 2628-2632. 10.21437/Interspeech.2023-1929. 
\cvitem{2023}{\scriptsize{Jay Kejriwal, Stefan Benus, Lina Rojas-Barahona}. \textbf{\em{Unsupervised Auditory and Semantic Entrainment Models with Deep Neural Networks.}} Proceedings of the 24th INTERSPEECH Conference. \textbf{INTERSPEECH}, Dublin, Ireland 2023}
\noindent \cvitem{.}{\scriptsize{Thibault Cordier, Tanguy Urvoy, Fabrice Lefevre, Lina Rojas-Barahona}. \textbf{\em{Few-Shot Structured Policy Learning for Multi-Domain and Multi-Task Dialogues.}} Proceedings of the Findings of The 17th Conference of the European Chapter of the Association for Computational Linguistics. \textbf{EACL}, Dubrovnik, Croatia 2023}
\noindent \cvitem{.}{\scriptsize{Sebastien Montella, Alexis Nasr, Johannes Heinecke, Frederic Bechet, Lina Rojas-Barahona}. \textbf{\em{Investigating the Effect of Relative Positional Embeddings on AMR-to-Text Generation with Structural Adapters.}} Proceedings of The 17th Conference of the European Chapter of the Association for Computational Linguistics. \textbf{EACL}, Dubrovnik 2023}
\noindent \cvitem{2022}{\scriptsize{Thibault Cordier, Tanguy Urvoy, Fabrice Lefevre, Lina Rojas-Barahona}. \textbf{\em{Graph Neural Network Policies and Imitation Learning for Multi-Domain Task-Oriented Dialogues.}} Proceedings of the Annual Meeting of the Special Interest Group on Discourse and Dialogue. \textbf{SIGDIAL}, Edinburgh 2022}

\noindent \cvitem{.}{\scriptsize{Leo Jacqmin, Lina Rojas-Barahona, Benoit Favre}. \textbf{\em{" Do you follow me?": A Survey of Recent Approaches in Dialogue State Tracking.}} Proceedings of the Annual Meeting of the Special Interest Group on Discourse and Dialogue. \textbf{SIGDIAL}, Stockholm, Edinburgh 2022}
\noindent \cvitem{.}{\scriptsize{Gwénolé Lecorvé, Morgan Veyret, Quentin Brabant, and Lina M. Rojas-Barahona.} \textbf{\em{SPARQL-to-Text Question Generation for Knowledge-Based Conversational Applications.}} Proceedings of the 2nd Conference of the Asia-Pacific Chapter of the Association for Computational Linguistics and the 12th International Joint Conference on Natural Language Processing. \textbf{AACL-IJCNLP} 2022}
\noindent \cvitem{.}{\scriptsize{Quenting Brabant, Gwenole Lecorve, Lina Rojas-Barahona}. \textbf{\em{Coqar: Question rewriting on CoQA.}} Proceedings of the Thirteenth Language Resources and Evaluation Conference. \textbf{LREC}, Marseille France 2022}
\noindent \cvitem{.}{\scriptsize{Frédéric Béchet, Ludivine Robert, Lina Rojas-Barahona and Géraldine Damnati.} \textbf{\em{Calor-Dial : a corpus for Conversational Question Answering on French encyclopedic documents.}} Joint Conference of the Information Retrieval Communities in Europe \textbf{CIRCLE} 2022 }  
\noindent \cvitem{2021}{\scriptsize{Sebastien Montella, Lina Rojas-Barahona, Johannes Heinecke}. \textbf{\em{Hyperbolic temporal knowledge graph embeddings with relational and time curvatures.}} Findings of the Association for Computational Linguistics: \textbf{ACL-IJCNLP 2021}}

\noindent \cvitem{2019}{\scriptsize{Lina Rojas-Barahona, Pascal Bellec, Benoit Besset, Martinho Dos-Santos, Johannes Heinecke,  Munshi Asadullah, Olivier Le-Blouch, Jean Y. Lancien,Géraldine Damnati, Emmanuel Mory and Frédéric Herledan}. \textbf{\em{Spoken Conversational Search for General Knowledge.}} Proceedings of the Annual Meeting of the Special Interest Group on Discourse and Dialogue. \textbf{SIGDIAL}, Stockholm, Sweden 2019}
%
\noindent \cvitem{.}{\scriptsize{Jean-Leon Bouraoui, Sonia Le Meitour, Romain Carbou, Lina M. Rojas Barahona, and Vincent Lemaire}. \textbf{\em{Graph2bots, unsupervised assistance for designing chatbots.}}Proceedings of the Annual Meeting of the Special Interest Group on Discourse and Dialogue. \textbf{SIGDIAL}, Stockholm, Sweden 2019}

\noindent \cvitem{2018}{\scriptsize{Stefan Ultes,Pawel Budzianowski,I\'nigo Casanueva,LinaRojas-Barahona, Bo-Hsiang Tseng, Yen-Chen Wu, Steve Young and Milica Gasic. \textbf{\em{Addressing Objects and Their Relations: The Conversational Entity Dialogue Model.}} Proceedings of the SIGDIAL Conference, Mebourne Australia 2018}}

\noindent \cvitem{2017}{\scriptsize{S. Ultes, L. Rojas-Barahona, P. Su, D. Vandyke, D. Kim, I. Casanueva, P. Budzianowski, T. Wen, M. Gašić and S. Young. \textbf{\em{PyDial: A Multi-domain Statistical Dialogue System Toolkit.}} Proceedings of the Meeting of the Association for Computational Linguistics. \textbf{ACL}, Vancouver, August 2017}}
\noindent \cvitem{.}{\scriptsize{Stefan Ultes, Paweł Budzianowski, Iñigo Casanueva, Nikola Mrkšić, Lina M. Rojas Barahona, Pei-Hao Su, Tsung-Hsien Wen, Milica Gasic and Steve Young. \textbf{\em{Reward-Balancing for Statistical Spoken Dialogue Systems using Multi-objective Reinforcement Learning.}} Proceedings of the 18th Meeting of the Special Interest Group in Discourse and Dialogue, \textbf{SIGDIAL}. Saarbrücken, August 2017.}}

\noindent \cvitem{.}{\scriptsize{Kyusong Lee, Tiancheng Zhao, Yulun Du, Edward Cai, Allen Lu, Eli Pincus, David Traum, Stefan Ultes, Lina M. Rojas-Barahona, Milica Gasic, Steve Young and Maxine Eskenazi.} \textbf{\em{Dialport, gone live: an update after a year of development.}} Proceedings of the 18th Meeting of the Special Interest Group in Discourse and Dialogue, \textbf{SIGDIAL}. Saarbrücken, August 2017.} 

\noindent \cvitem{.}{\scriptsize{Pawel Budzianowski, Stefan Ultes, Pei-Hao Su, Nikola Mrksic, Tsung-Hsien Wen, Iñigo Casanueva, Lina M. Rojas-Barahona, and Milica Gasic.} \textbf{ \em{ Sub-domain Modelling for Dialogue Management with Hierarchical Reinforcement Learning.}} Proceedings of the 18th Meeting of the Special Interest Group in Discourse and Dialogue, \textbf{SIGDIAL}. Saarbrücken, August 2017.}

\noindent \cvitem{.}{\scriptsize{S. Ultes, P. Budzianowski, I. Casanueva, N. Mrksic, L. Rojas-Barahona, P.-H. Su, T.-H. Wen, M. Gasic and S. Young. \textbf{\em{Domain-independent User Satisfaction Reward Estimation for Dialogue Policy Learning.}} \textbf{INTERSPEECH} 2017. Stockholm Sweden.}}

\noindent \cvitem{.}{\scriptsize{T.-H. Wen, D. Vandyke, N. Mrksic, M. Gasic, L. Rojas-Barahona, P.-H. Su, S. Ultes and S. Young. \textbf{\em{A Network-based End-to-End Trainable Task-oriented Dialogue System.}.} \textbf{EACL} 2017, Valencia, Spain.}}



\noindent \cvitem{2016}{\scriptsize{L. Rojas-Barahona, M. Gasic, N. Mrksic, P.-H. Su, S. Ultes, T.-H. Wen and S. Young. \textbf{\em{Exploiting Sentence and Context Representations in Deep Neural Models for Spoken Language Understanding.}.} \textbf{COLING} 2016, Osaka, Japan.}}
\noindent \cvitem{.}{\scriptsize{T.-H. Wen, M. Gasic, N. Mrksic, L. Rojas-Barahona, P.-H. Su, S. Ultes, D. Vandyke and S. Young (2016). \textbf{\em{Conditional Generation and Snapshot Learning in Neural Dialogue Systems.}} \textbf{EMNLP} 2016. Austin, Texas. }}
\noindent \cvitem{.}{\scriptsize{P-H. Su, M. Gasic, N. Mrksic, L. Rojas-Barahona, S. Ultes, D. Vandyke, T-H. Wen, and S. Young (2016). \textbf{\em{On-line Active Reward Learning for Policy Optimisation in Spoken Dialogue Systems.}} \textbf{ACL} 2016, Berlin.[Best student paper]}}
\noindent \cvitem{.}{\scriptsize{T.-H. Wen, M. Gasic, N. Mrksic, L. Rojas-Barahona, P.-H. Su, D. Vandyke and S. Young (2016). \textbf{\em{Multi-domain Neural Network Language Generation for Spoken Dialogue Systems.}} \textbf{NAACL HLT} 2016, San Diego.}}
\noindent \cvitem{.}{\scriptsize{N. Mrksic, D. O Seaghdha, B. Thomson, M. Gasic, L. Rojas-Barahona, P.-H. Su, D. Vandyke, T.-H. Wen and S. Young (2016). \textbf{\em{Counter-fitting Word Vectors to Linguistic Constraints.} NAACL HLT} 2016, San Diego.}}
\noindent \cvitem{2015}{\scriptsize{Lina M. Rojas-Barahona and Christophe Cerisara. \textbf{\em{Weakly Supervised Discriminative Training of Linear Models for Natural Language Processing.}} In proceedings of the 3rd International Conference on Statistical Language and Speech Processing. \textbf{SLSP} 2015. Budapest, Hungary.}}
\noindent \cvitem{.}{\scriptsize{Lina M. Rojas-Barahona and Christophe Cerisara. \em{Enhanced discriminative models with tree kernels and unsupervised training for entity detection.} In proceedings of the 6th International Conference on Information Systems and Economic Intelligence. \textbf{SIIE} 2015. Hammamet,Tunisia.}}

\noindent \cvitem{2014}{\scriptsize{Lina M. Rojas-Barahona and Christophe Cerisara. \textbf{\em{Bayesian Inverse Reinforcement Learning for Modeling Conversational Agents in a Virtual Environment}}.In proceedings of the 15th International Conference on Intelligent Text Processing and Computational Linguistics, LNCS Springer. \textbf{CICLING} 2014, Kathmandu, Nepal.}}
\noindent \cvitem{2013}{\scriptsize{Claire Gardent and Lina Maria Rojas-Barahona. \textbf{\em{Using Paraphrases and Lexical Semantics to Improve the Accuracy and the Robustness of Supervised Models in Situated Dialogue Systems.}}
In proceedings of the 2013 Conference on Empirical Methods in Natural Language Processing, \textbf{EMNLP} 2013, Seattle, USA.}}
\noindent \cvitem{.}{\scriptsize{Alejandra Lorenzo, Lina Rojas-Barahona and Christophe Cerisara. \textbf{\em{Unsupervised structured semantic inference for spoken dialog reservation tasks. }}
Proceedings of the 14th annual SIGdial Meeting on Discourse and Dialogue. \textbf{SIGDIAL} 2013, Metz France.}}
\noindent \cvitem{.}{\scriptsize{Claire Gardent, Alejandra Lorenzo, Laura Perez-Beltrachini and Lina M. Rojas-Barahona. \textbf{\em{Weakly and Strongly Constrained Dialogues for Language Learning.}} Proceedings of the 14th annual SIGdial Meeting on Discourse and Dialogue. \textbf{SIGDIAL 2013}, Metz France.}}

\noindent \cvitem{2012}{\scriptsize{Lina Maria Rojas-Barahona, Alejandra Lorenzo and Claire Gardent. \textbf{\em{An End-to-End Evaluation of Two Situated Dialog Systems.}}
Proceedings of the 13th annual SIGdial Meeting on Discourse and Dialogue. \textbf{SIGDIAL} 2012, Seoul Korea.}}
\noindent \cvitem{.}{\scriptsize{Lina Maria Rojas-Barahona, Alejandra Lorenzo and Claire Gardent. \textbf{\em{Building and Exploiting a Corpus of Dialog Interactions between French Speaking Virtual and Human Agents.}}
\textbf{LREC} 2012, The eighth international conference on Language Resources and Evaluation. , May 2012, Istanbul, Turkey.}}
\noindent \cvitem{}{\scriptsize{Fabrice Lef{\`e}vre; Djamel Mostefa; Laurent Besacier; Yannick Est{\`e}ve; Matthieu Quignard; Nathalie Camelin; Benoit Favre; Bassam Jabaian; Lina Maria Rojas-Barahona. \textbf{\em{Leveraging study of robustness and portability of spoken language understanding systems across languages and domains: the PORTMEDIA corpora.}} \textbf{LREC} 2012, The International Conference on Language Resources and Evaluation, May 2012, Istanbul, Turkey.}}
\noindent \cvitem{2011}{\scriptsize{Lina Maria Rojas-Barahona and Matthieu Quignard. \textbf{\em{An Incremental Architecture for the Semantic Annotation of Dialogue Corpora with High-Level Structures. A case study for the MEDIA corpus.}}
Proceedings of the 12th annual SIGdial Meeting on Discourse and Dialogue. \textbf{SIGDIAL} 2011, Portland Oregon. June 2011.}}

\noindent \cvitem{2010}{\scriptsize{C. Larizza, M. Gabetta, L. Rojas Barahona, G. Milani, E. Guaschino, G. Sances, C. Cereda, R. Bellazzi. \textbf{\em{Extraction of Clinical Information from Clinical Reports: an Application to the Study of Medication Overuse Headaches in Italy.}} In proceedings of the \textbf{AMIA} Summit on Translational Bioinformatics, San Francisco, March 2010.}}
\noindent \cvitem{2009}{\scriptsize{Silvana Quaglini, Toni Giorgino, Lina M. Rojas-Barahona, Ezio Caffi, Mauro De Vito, Alessandra Persico and Anna cavallini. \textbf{\em{An Automated Voice Response System for Anticoagulant Therapy Management.}} Proceedings of the XXII International Conference of the European Federation for Medical Informatics, \textbf{MIE09}, (2009)}}
\noindent \cvitem{.}{\scriptsize{Lina Maria Rojas-Barahona, Silvana Quaglini and Mario Stefanelli. \textbf{\em{HomeNL: Homecare Assistance in Natural Language. An Intelligent Conversational Agent for Hypertensive Patients Management.} }Proceedings of the 12th Conference on Artificial Intelligence in Medicine, \textbf{AIME09}  ,ed Carlo Combi, Yuval Shahar, Ameen Abu-Hanna. LNCS Springer (2009)}}

\noindent \cvitem{2007}{\scriptsize{L. M. Rojas-Barahona, T. Giorgino.} \textbf{\em{AdaRTE: Adaptable Dialogue Architecture and Runtime Engine. A new architecture for health-Care dialogue systems. Proceedings of 12th World Congress on Health (Medical) Informatics (\textbf{MEDINFO} 2007).}}}

\subsection{Workshops}

\cvitem{2022}{\scriptsize{Sebastien Montella, Lina Rojas-Barahona, Frederic Bechet, Johannes Heinecke, and Alexis Nasr.} \textbf{\em{Transfer Learning and Masked Generation for Answer Verbalization.}} Proceedings of the Workshop on Structured and Unstructured Knowledge Integration (SUKI) ACL 2022.}

\noindent \cvitem{2021}{\scriptsize{Quentin Brabant, Lina Rojas-Barahona, Claire Gardent}. \textbf{\em{Active Learning and Multi-label Classification for Ellipsis and Coreference Detection in Conversational Question-Answering.}}. \textbf{IWSDS 2021}.}
\noindent \cvitem{2020}{\scriptsize{Lina Rojas-Barahona}. \textbf{\em{Is the User Enjoying the Conversation? A Case Study on the Impact on the Reward Function.}} NeurIPS Workshop: Human in the Loop Dialogue Systems, Proceedings of the 34st Conference on Neural Information Processing Systems (\textbf{NeurIPS 2020})}
\noindent \cvitem{.}{\scriptsize{Thibault Cordier, Tanguy Urvoy, Lina Rojas-Barahona, Fabrice Lefevre}. \textbf{\em{Diluted near-optimal expert demonstrations for guiding dialogue stochastic policy optimisation}} NeurIPS Workshop: Human in the Loop Dialogue Systems, Proceedings of the 34st Conference on Neural Information Processing Systems (\textbf{NeurIPS 2020})}
\noindent \cvitem{.}{\scriptsize{S.ebastien Montella, Betty Fabre, Tanguy Urvoy, Johannes Heinecke, Lina Rojas-Barahona.} \textbf{ \em{Denoising pre-training and data augmentation strategies for enhanced RDF verbalization with transformers.}} Proceedings of the 3rd International Workshop on Natural Language Generation from the Semantic Web (WebNLG+) 2020}
\noindent \cvitem{2018}{\scriptsize{Lina Rojas-Barahona,Bo-Hsiang Tseng, Yinpei Dai, Clare Mansfield, Osman Ramadan, Stefan Ultes, Michael Crawford	and Milica Gašić. \textbf{\em{Deep learning for language understanding of mental health concepts derived from Cognitive Behavioural Therapy.}} Proceedings of the The Ninth International Workshop on Health Text Mining and Information Analysis, 2018}}
\noindent \cvitem{2017}{\scriptsize{K. Lee, T. Zhao, S. Ultes, L. Rojas-Barahona, E. Pincus, D. Traum and M. Eskenazi. \textbf{\em{An assessment framework for DialPort.}} Proceedings of the 8th International Workshop On Spoken Dialogue Systems, \textbf{IWSDS}, Farmington, USA, June 2017}}
\noindent \cvitem{.}{\scriptsize{I. Casanueva, P. Budzianowski, P.-H. Su, N. Mrksic, T.-H. Wen, S. Ultes, L. Rojas-Barahona, S. Young and M. Gasic. \textbf{\em{A Benchmarking Environment for Reinforcement Learning Based Task Oriented Dialogue Management.}} Deep Reinforcement Learning Symposium at the 31st Conference on Neural Information Processing Systems (\textbf{NIPS 2017}), \textbf{IWSDS}, Farmington, USA, June 2017}}
%31st Conference on Neural Information Processing Systems (NIPS 2017)
\noindent \cvitem{2015}{\scriptsize{T.-H. Wen, M. Gasic, N. Mrksic, L. Rojas-Barahona, P.-H. Su, D. Vandyke and S. Young (2015). \textbf{\em{Toward Multi-domain Language Generation using Recurrent Neural Networks.}} Workshop on Machine Learning for Spoken Language Understanding and Interaction \textbf{NIPS 2015}, Montreal.}}
\noindent \cvitem{2012}{\scriptsize{Lina Maria Rojas-Barahona and Claire Gardent. \em{What Should I Do Now? Supporting Progress in a Serious Game.} Proceedings of the 16th workshop on the semantics and pragmatics of dialogue. \textbf{SEINEDIAL 2012}, Paris France.}}
\noindent \cvitem{2011}{\scriptsize{Lina Maria Rojas-Barahona and Thierry Bazillon and Matthieu Quignard and Fabrice Lefevre. \textbf{\em{Using MMIL for the High Level Semantic Annotation of the French MEDIA Dialogue Corpus.}} Proceedings of the 9th International Conference on Computational Semantics, \textbf{IWCS}. Oxford, January 2011.}}
\noindent \cvitem{2010}{\scriptsize{Alexandre Denis, Lina M. Rojas-Barahona and Matthieu Quignard. Extending MMIL Semantic Representation: Experiments in Dialogue Systems and Semantic Annotation of Corpora. In proceedings of the Fifth Joint ISO-ACL/SIGSEM Workshop on Interoperable Semantic Annotation (\textbf{ISA-5}), Hong Kong, January 2010.}}
\noindent \cvitem{2007}{\scriptsize{L.M Rojas-Barahona. \textbf{\em{Adapting combinatory categorial grammars in a framework for health care dialogue systems.}} \textbf{Decalog} 2007: Proceedings of the 11th Workshop on the Semantics and Pragmatics of Dialogue, 2007.}}
\noindent \cvitem{}{\scriptsize{L.M Rojas-Barahona, T. Giorgino. AdaRTE: An extensible and adaptable architecture for dialog systems. Bridging the gap: academic and industrial research in dialog technologies \textbf{workshop proceedings, ed NAACL-HLT}, 2007.}}

\subsection{French Conferences}
\cvitem{2022}{\scriptsize{Thibault Cordier, Fabrice Lefèvre, Tanguy Urvoy, Lina Maria Rojas-Barahona.} \textbf{ \em{Et la robustesse ?...  Comment les stratégies de dialogue par apprentissage structuré résistent aux bruits des entrées ?.}} Proc. XXXIVe Journées d'Études sur la Parole -- JEP 2022}
%Robustesse et portabilités multilingue et multi-domaines des systèmes de compréhension de la parole: les corpus du projet PORTMEDIA
